Facing the Music: Tackling Singing Voice Separation in Cinematic Audio Source Separation

Cinematic audio source separation (CASS), as a standalone problem of extracting individual stems from their mixture, is a fairly new subtask of audio source separation. A typical setup of CASS is a three-stem problem, with the aim of separating the mixture into the dialogue (DX), music (MX), and effects (FX) stems. Given the creative nature of cinematic sound production, however, several edge cases exist; some sound sources do not fit neatly in any of these three stems, necessitating the use of additional auxiliary stems in production. One very common edge case is the singing voice in film audio, which may belong in either the DX or MX or neither, depending heavily on the cinematic context. In this work, we demonstrate a very straightforward extension of the dedicated-decoder Bandit and query-based single-decoder Banquet models to a four-stem problem, treating non-musical dialogue, instrumental music, singing voice, and effects as separate stems. Interestingly, the query-based Banquet model outperformed the dedicated-decoder Bandit model. We hypothesized that this is due to a better feature alignment at the bottleneck as enforced by the band-agnostic FiLM layer. Dataset and model implementation will be made available at https://github.com/kwatcharasupat/source-separation-landing.

==> tables/query-vdb.tex <==
\begin{tabularx}{\columnwidth}{cCC
    S[table-format=-2.1]
    S[table-format=-2.1]
    S[table-format=-2.1]
    S[table-format=-2.1]}
        \toprule
        % \multicolumn{2}{c}{\textbf{Encoder}}
        % & & \multicolumn{4}{c}{\textbf{Median SNR (dB)}}\\
        % \cmidrule{1-2}
        % \cmidrule{4-7}
        \textbf{Pretrained Enc.} &\textbf{FE} & \textbf{DA} & {\textbf{Female Vox}} & {\textbf{Male Vox}} & {\textbf{Drums}} & {\textbf{Bass}} \\
        \midrule
        N & N & N & 8.3 & 7.2 & 9.4 & 9.4 \\
        % \midrule
        Y & Y & N & 9.8 & 7.6 & 9.9 & 10.2 \\
        Y & N & N & 9.8 & \bfseries 8.0 & 9.3 & 9.8 \\
        Y & N & Y & \bfseries 10.2 & \bfseries 8.0 & \bfseries 10.1 & \bfseries 10.8 \\
        \bottomrule
    \end{tabularx}

==> tables/query-vdbgp-coarse.tex <==

\begin{tabularx}{\columnwidth}{
    X
    ccc
    S[table-format=2.1]
        S[table-format=2.1]
        S[table-format=2.1]
    S[table-format=2.1]
        S[table-format=2.1]
        S[table-format=2.1]
}
    \toprule
    % \cmidrule(lr){20-22}
    % \cmidrule(lr){23-25}
    % \cmidrule(lr){26-28}
    % \cmidrule(lr){29-31}
    \textbf{Model} &
    \textbf{FE}  & 
    \textbf{DA} &
    \textbf{BS} & 
    {\textbf{Vox}} &
    {\textbf{Lead Vox}} &
    {\textbf{Drums}} &
    {\textbf{Bass}} &
    {\textbf{Guitar}} &
    {\textbf{Piano}} \\
\midrule
Banquet & Y & N & N & \bfseries 8.0 & 7.9 & 9.8 & 10.5 & 2.3 & 0.8 \\
& &  & Y & 7.9 & 7.7 & 9.6 & 10.5 & 2.2 & 0.9 \\
\cmidrule{2-10}
&N & N & N & 7.4 & \bfseries 8.0 & 9.6 & 10.6 & 3.0 & 2.3 \\
& &  & Y & 7.6 & 7.7 & 9.3 & 10.2 & 2.9 & \bfseries 2.5 \\
\cmidrule{3-10}
& & Y & N & 7.8 & 7.9 & \bfseries 10.1 & 10.9 & 3.2 & 2.2 \\
& &  & Y & 7.6 & 7.9 & 9.5 & \bfseries 11.0 & \bfseries 3.3 & \bfseries 2.5 \\
 \midrule
\multicolumn{4}{l}{HT-Demucs (\textsc{vdbgpo})} & 
    \bfseries 8.9 & \multicolumn{1}{c}{---} & \bfseries 11.6 & \bfseries 12.4 & 2.4 & 1.7 
\\
\multicolumn{4}{l}{Spleeter (\textsc{vdbpo})} & 
    7.0 & \multicolumn{1}{c}{---} & 6.9 & 6.7 & \multicolumn{1}{c}{---} & 0.7
\\
\midrule
\multicolumn{4}{l}{Oracle IRM} & 10.0 & \multicolumn{1}{c}{---} & 9.6 & 7.8 & 5.2 & 5.0\\
\bottomrule
\end{tabularx}

==> tables/query-vdbgp-old.tex <==
\begin{tabularx}{\textwidth}{
    CCCC@{\hspace{6pt}}
    S[table-format=2.1]
        S[table-format=2.1]
        S[table-format=2.1]
        @{\hspace{6pt}}
    S[table-format=2.1]
        S[table-format=2.1]
        S[table-format=2.1]
        @{\hspace{6pt}}
    S[table-format=2.1]
        S[table-format=2.1]
        S[table-format=2.1]
        @{\hspace{6pt}}
    S[table-format=2.1]
        S[table-format=2.1]
        S[table-format=2.1]
        @{\hspace{6pt}}
    S[table-format=2.1]
        S[table-format=2.1]
        S[table-format=2.1]
        @{\hspace{6pt}}
    S[table-format=2.1]
        S[table-format=2.1]
        S[table-format=2.1]
        @{\hspace{6pt}}
    S[table-format=2.1]
        S[table-format=2.1]
        S[table-format=2.1]
        @{\hspace{6pt}}
    S[table-format=-2.1]
        S[table-format=2.1]
        S[table-format=2.1]
        @{\hspace{6pt}}
    S[table-format=-2.1]
        S[table-format=2.1]
        S[table-format=2.1]
}
    \toprule
     &
    % \multicolumn{2}{c}{\textbf{Data}} & &
    &&&
    \multicolumn{3}{c}{\textbf{Female Vox}} & 
    \multicolumn{3}{c}{\textbf{Male Vox}} & 
    \multicolumn{3}{c}{\textbf{Drums}} & 
    \multicolumn{3}{c}{\textbf{Bass}} & 
    \multicolumn{3}{c}{\textbf{Acoust. Gtr.}} & 
    \multicolumn{3}{c}{\textbf{Clean E. Gtr.}} & 
    \multicolumn{3}{c}{\textbf{Dist. E. Gtr.}} & 
    \multicolumn{3}{c}{\textbf{Grand Piano}} & 
    \multicolumn{3}{c}{\textbf{E. Piano}}\\
    % \cmidrule(lr){1-1}
    % \cmidrule(lr){2-3}
    % \cmidrule{5-13}
    \cmidrule(lr){5-7}
    \cmidrule(lr){8-10}
    \cmidrule(lr){11-13}
    \cmidrule(lr){14-16}
    \cmidrule(lr){17-19}
    \cmidrule(lr){20-22}
    \cmidrule(lr){23-25}
    \cmidrule(lr){26-28}
    \cmidrule(lr){29-31}
    \textbf{FE}  & 
    \textbf{DA} &
    \textbf{BS} & 
    \textbf{SSQ} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} \\
\midrule
% Y & N & N & N & 7.2 & 9.6 & 12.8 & 6.4 & 7.6 & 9.9 & 8.2 & 9.8 & 11.8 & 8.1 & 10.1 & 12.1 & 0.4 & 1.5 & 2.4 & 0.1 & 0.5 & 1.6 & 0.6 & 2.7 & 4.9 & -0.3 & 0.8 & 2.4 & 0.2 & 0.5 & 0.9 \\
%  &  &  & Y & \bfseries 7.3 & 9.7 & 12.8 & 6.7 & 7.6 & 9.9 & 8.2 & 9.8 & 11.8 & 8.0 & 10.1 & 12.1 & 0.4 & 1.5 & 2.4 & 0.2 & 0.6 & 1.6 & 0.6 & 2.6 & 4.8 & -0.3 & 0.8 & 2.4 & 0.3 & 0.5 & 0.7 \\
%  \cmidrule(){3-31}
%  &  & Y & N & 7.0 & 9.4 & 12.2 & 6.5 & 7.4 & 9.8 & 8.1 & 9.6 & 11.5 & 7.9 & 10.2 & 11.9 & 0.3 & 1.5 & 2.5 & 0.1 & 0.5 & 1.7 & 0.5 & 2.7 & 4.9 & -0.2 & 1.0 & 2.2 & 0.1 & 0.5 & 0.8 \\
%  &  &  & Y & 6.9 & 9.5 & 12.3 & 6.7 & 7.4 & 9.8 & 8.1 & 9.6 & 11.5 & 7.7 & 10.3 & 11.9 & 0.3 & 1.5 & 2.5 & 0.1 & 0.5 & 1.8 & 0.5 & 2.7 & 4.9 & -0.2 & 0.9 & 2.2 & 0.3 & 0.5 & 0.9 \\
% \midrule
N & N & N & N & 5.5 & 9.6 & 13.2 & 6.7 & \bfseries 7.9 & 10.0 & 8.0 & 9.6 & 11.6 & 7.9 & 9.9 & 12.0 & 0.9 & \bfseries 1.8 & 3.6 & 0.2 & 0.7 & 2.4 & 0.9 & 2.4 & 5.3 & 0.7 & 2.3 & 2.9 & 0.0 & 0.6 & 0.7 \\
 &  &  & Y & 5.6 & 9.6 & 13.2 & 6.7 & \bfseries 7.9 & 10.0 & 8.0 & 9.6 & 11.6 & 7.9 & 9.9 & 12.0 & 0.9 & \bfseries 1.8 & 3.7 & 0.2 & 0.9 & 2.6 & 0.9 & 2.4 & 5.3 & 0.7 & 2.2 & 3.0 & 0.0 & 0.8 & 1.5 \\
  \cmidrule(){3-31}
 &  & Y & N & 6.1 & 9.6 & 13.1 & 6.8 & 7.7 & 9.7 & 7.8 & 9.3 & 11.3 & 7.6 & 10.0 & 11.5 & 0.8 & \bfseries 1.8 & 3.6 & 0.2 & 0.8 & 2.5 & 1.0 & 2.5 & \bfseries 5.4 & \bfseries 0.8 & 2.5 & 3.1 & -0.1 & 0.7 & 0.8 \\
 &  &  & Y & 6.1 & 9.6 & 13.1 & 6.8 & 7.7 & 9.7 & 7.8 & 9.3 & 11.3 & 7.6 & 10.0 & 11.5 & 0.8 & \bfseries 1.8 & 3.7 & -0.0 & 0.9 & 2.7 & \bfseries 1.2 & 2.5 & \bfseries 5.4 & \bfseries 0.8 & 2.5 & 3.1 & -0.6 & 0.8 & 1.8 \\
 \cmidrule(){2-31}
 & Y & N & N & 5.5 & \bfseries 10.1 & 13.0 & \bfseries 6.9 & \bfseries 7.9 & \bfseries 10.2 & \bfseries 8.5 & \bfseries 10.1 & \bfseries 12.3 & \bfseries 8.4 & \bfseries 10.7 & \bfseries 13.2 & \bfseries 1.2 & 1.7 & 4.5 & 0.2 & 0.9 & \bfseries 3.0 & 0.9 & 2.8 & 4.7 & \bfseries 0.8 & \bfseries 2.8 & \bfseries 3.2 & 0.1 & 0.5 & 0.9 \\
 &  &  & Y & 5.5 & \bfseries 10.1 & 13.1 & \bfseries 6.9 & \bfseries 7.9 & \bfseries 10.2 & \bfseries 8.5 & \bfseries 10.1 & \bfseries 12.3 & \bfseries 8.4 & \bfseries 10.7 & \bfseries 13.2 & \bfseries 1.2 & 1.7 & \bfseries 4.6 & 0.2 & \bfseries 1.1 & 2.7 & 0.9 & 2.8 & 4.7 & \bfseries 0.8 & 2.4 & 3.1 & -0.1 & 0.6 & 0.9 \\
 \cmidrule(){3-31}
 &  & Y & N & 5.5 & \bfseries 10.1 & \bfseries 13.5 & 6.5 & 7.8 & 10.0 & 8.3 & 9.5 & 11.8 & \bfseries 8.4 & 10.3 & 12.1 & 1.1 & 1.7 & 3.9 & 0.0 & 0.4 & 2.7 & 0.9 & \bfseries 3.0 & 4.9 & \bfseries 0.8 & 2.6 & \bfseries 3.2 & 0.2 & 0.5 & 0.9 \\
 &  &  & Y & 5.5 & \bfseries 10.1 & \bfseries 13.5 & 6.5 & 7.8 & 10.0 & 8.3 & 9.5 & 11.8 & 7.8 & 10.3 & 12.1 & 1.0 & 1.7 & 3.9 & \bfseries 0.3 & 0.6 & 2.7 & 0.6 & \bfseries 3.0 & 4.8 & \bfseries 0.8 & 2.5 & \bfseries 3.2 & \bfseries 0.6 & \bfseries 0.9 & \bfseries 2.1 \\
%  \midrule
%  &&&& \multicolumn{3}{c}{\textbf{Vocals}} &
%  &&& \multicolumn{3}{c}{\textbf{Drums}} &
%  \multicolumn{3}{c}{\textbf{Bass}} &
%  &&& \multicolumn{3}{c}{\textbf{Guitar}} &
%  &&& \multicolumn{3}{c}{\textbf{Piano}}
%  \\
%     \cmidrule(lr){5-7}
%     % \cmidrule(lr){8-10}
%     \cmidrule(lr){11-13}
%     \cmidrule(lr){14-16}
%     % \cmidrule(lr){17-19}
%     \cmidrule(lr){20-22}
%     % \cmidrule(lr){23-25}
%     \cmidrule(lr){26-28}
%     % \cmidrule(lr){29-31}
% \multicolumn{4}{l}{HT-Demucs (VDBGPO)} & 
%     8.3 & 9.0 & 10.3 & &&&
%     \textbf{\textit{9.0}} & \textbf{\textit{11.6}} & \textbf{\textit{12.8}} & 
%     \textbf{\textit{11.2}} & \textbf{\textit{12.4}} & \textbf{\textit{14.1}} & &&& 
%     1.5 & 2.4 & 4.4 & &&&
%     0.2 & 1.7 & 2.3
% \\
% \multicolumn{4}{l}{Spleeter (VDBPO)} & 
%     6.0 & 7.0 & 7.7 & &&&
%     5.6 & 6.9 & 8.6 & 
%     5.2 & 6.7 & 8.8 & &&& 
%     &&& &&&
%     0.0 & 0.7 & 1.7
% \\
% \midrule

% \multicolumn{4}{l}{Oracle IBM} & 10.6 & 12.0 & 12.4 & 8.6 & 9.9 & 10.8 & 7.7 & 9.4 & 10.3 & 6.6 & 7.9 & 9.9 & 3.4 & 4.3 & 6.2 & 3.9 & 5.8 & 7.3 & 5.0 & 6.1 & 7.5 & 3.4 & 4.3 & 6.1 & 4.1 & 5.2 & 5.5 \\

% \multicolumn{4}{l}{Oracle IRM} & 10.0 & 11.3 & 11.9 & 8.0 & 9.3 & 10.1 & 7.0 & 8.5 & 9.5 & 6.0 & 7.4 & 9.3 & 3.0 & 4.2 & 5.7 & 3.5 & 5.6 & 6.9 & 4.6 & 5.8 & 6.9 & 3.1 & 4.4 & 5.8 & 3.9 & 4.9 & 5.2 \\
\bottomrule
\end{tabularx}

==> tables/query-vdbgp.tex <==
\begin{tabularx}{\textwidth}{
    cccC@{\hspace{6pt}}
    %%%% 
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        @{\hspace{6pt}}
    %%%% 
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        @{\hspace{6pt}}
    %%%% 
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        @{\hspace{6pt}}
    %%%% 
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        @{\hspace{6pt}}
    %%%% 
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        @{\hspace{6pt}}
    %%%% 
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        @{\hspace{6pt}}
    %%%% 
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        @{\hspace{6pt}}
    %%%% 
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        @{\hspace{6pt}}
    %%%% 
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        P{min=-0.6, max=13.5, first color=yellow, second color=orange}{table-format=2.1}
        @{\hspace{6pt}}
}
    \toprule
     &
    % \multicolumn{2}{c}{\textbf{Data}} & &
    &&&
    \multicolumn{3}{c}{\textbf{Female Vox}} & 
    \multicolumn{3}{c}{\textbf{Male Vox}} & 
    \multicolumn{3}{c}{\textbf{Drums}} & 
    \multicolumn{3}{c}{\textbf{Bass Gtr.}} & 
    \multicolumn{3}{c}{\textbf{Acoust. Gtr.}} & 
    \multicolumn{3}{c}{\textbf{Clean E. Gtr.}} & 
    \multicolumn{3}{c}{\textbf{Dist. E. Gtr.}} & 
    \multicolumn{3}{c}{\textbf{Grand Piano}} & 
    \multicolumn{3}{c}{\textbf{E. Piano}}\\
    % \cmidrule(lr){1-1}
    % \cmidrule(lr){2-3}
    % \cmidrule{5-13}
    \cmidrule(lr){5-7}
    \cmidrule(lr){8-10}
    \cmidrule(lr){11-13}
    \cmidrule(lr){14-16}
    \cmidrule(lr){17-19}
    \cmidrule(lr){20-22}
    \cmidrule(lr){23-25}
    \cmidrule(lr){26-28}
    \cmidrule(lr){29-31}
    \textbf{FE}  & 
    \textbf{DA} &
    \textbf{BS} & 
    \textbf{STQ} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} &
    {\textbf{Q1}} &
        {\textbf{Q2}} &
        {\textbf{Q3}} \\
\midrule
Y & N & N & N & 7.2 & 9.6 & 12.8 & 6.4 & 7.6 & 9.9 & 8.2 & 9.8 & 11.8 & 8.1 & 10.1 & 12.1 & 0.4 & 1.5 & 2.4 & 0.1 & 0.5 & 1.6 & 0.6 & 2.7 & 4.9 & -0.3 & 0.8 & 2.4 & 0.2 & 0.5 & 0.9 \\
 &  &  & Y &  7.3 & 9.7 & 12.8 & 6.7 & 7.6 & 9.9 & 8.2 & 9.8 & 11.8 & 8.0 & 10.1 & 12.1 & 0.4 & 1.5 & 2.4 & 0.2 & 0.6 & 1.6 & 0.6 & 2.6 & 4.8 & -0.3 & 0.8 & 2.4 & 0.3 & 0.5 & 0.7 \\
 \cmidrule(){3-31}
 &  & Y & N & 7.0 & 9.4 & 12.2 & 6.5 & 7.4 & 9.8 & 8.1 & 9.6 & 11.5 & 7.9 & 10.2 & 11.9 & 0.3 & 1.5 & 2.5 & 0.1 & 0.5 & 1.7 & 0.5 & 2.7 & 4.9 & -0.2 & 1.0 & 2.2 & 0.1 & 0.5 & 0.8 \\
 &  &  & Y & 6.9 & 9.5 & 12.3 & 6.7 & 7.4 & 9.8 & 8.1 & 9.6 & 11.5 & 7.7 & 10.3 & 11.9 & 0.3 & 1.5 & 2.5 & 0.1 & 0.5 & 1.8 & 0.5 & 2.7 & 4.9 & -0.2 & 0.9 & 2.2 & 0.3 & 0.5 & 0.9 \\
\midrule
N & N & N & N & 5.5 & 9.6 & 13.2 & 6.7 &  7.9 & 10.0 & 8.0 & 9.6 & 11.6 & 7.9 & 9.9 & 12.0 & 0.9 &  1.8 & 3.6 & 0.2 & 0.7 & 2.4 & 0.9 & 2.4 & 5.3 & 0.7 & 2.3 & 2.9 & 0.0 & 0.6 & 0.7 \\
 &  &  & Y & 5.6 & 9.6 & 13.2 & 6.7 &  7.9 & 10.0 & 8.0 & 9.6 & 11.6 & 7.9 & 9.9 & 12.0 & 0.9 &  1.8 & 3.7 & 0.2 & 0.9 & 2.6 & 0.9 & 2.4 & 5.3 & 0.7 & 2.2 & 3.0 & 0.0 & 0.8 & 1.5 \\
  \cmidrule(){3-31}
 &  & Y & N & 6.1 & 9.6 & 13.1 & 6.8 & 7.7 & 9.7 & 7.8 & 9.3 & 11.3 & 7.6 & 10.0 & 11.5 & 0.8 &  1.8 & 3.6 & 0.2 & 0.8 & 2.5 & 1.0 & 2.5 &  5.4 &  0.8 & 2.5 & 3.1 & -0.1 & 0.7 & 0.8 \\
 &  &  & Y & 6.1 & 9.6 & 13.1 & 6.8 & 7.7 & 9.7 & 7.8 & 9.3 & 11.3 & 7.6 & 10.0 & 11.5 & 0.8 &  1.8 & 3.7 & -0.0 & 0.9 & 2.7 &  1.2 & 2.5 &  5.4 &  0.8 & 2.5 & 3.1 & -0.6 & 0.8 & 1.8 \\
 \cmidrule(){2-31}
 & Y & N & N & 5.5 &  10.1 & 13.0 &  6.9 &  7.9 &  10.2 &  8.5 &  10.1 &  12.3 &  8.4 &  10.7 &  13.2 &  1.2 & 1.7 & 4.5 & 0.2 & 0.9 &  3.0 & 0.9 & 2.8 & 4.7 &  0.8 &  2.8 &  3.2 & 0.1 & 0.5 & 0.9 \\
 &  &  & Y & 5.5 &  10.1 & 13.1 &  6.9 &  7.9 &  10.2 &  8.5 &  10.1 &  12.3 &  8.4 &  10.7 &  13.2 &  1.2 & 1.7 &  4.6 & 0.2 &  1.1 & 2.7 & 0.9 & 2.8 & 4.7 &  0.8 & 2.4 & 3.1 & -0.1 & 0.6 & 0.9 \\
 \cmidrule(){3-31}
 &  & Y & N & 5.5 &  10.1 &  13.5 & 6.5 & 7.8 & 10.0 & 8.3 & 9.5 & 11.8 &  8.4 & 10.3 & 12.1 & 1.1 & 1.7 & 3.9 & 0.0 & 0.4 & 2.7 & 0.9 &  3.0 & 4.9 &  0.8 & 2.6 &  3.2 & 0.2 & 0.5 & 0.9 \\
 &  &  & Y & 5.5 &  10.1 &  13.5 & 6.5 & 7.8 & 10.0 & 8.3 & 9.5 & 11.8 & 7.8 & 10.3 & 12.1 & 1.0 & 1.7 & 3.9 &  0.3 & 0.6 & 2.7 & 0.6 &  3.0 & 4.8 &  0.8 & 2.5 &  3.2 &  0.6 &  0.9 &  2.1 \\
%  \midrule
%  &&&& \multicolumn{3}{c}{\textbf{Vocals}} &
%  &&& \multicolumn{3}{c}{\textbf{Drums}} &
%  \multicolumn{3}{c}{\textbf{Bass}} &
%  &&& \multicolumn{3}{c}{\textbf{Guitar}} &
%  &&& \multicolumn{3}{c}{\textbf{Piano}}
%  \\
%     \cmidrule(lr){5-7}
%     % \cmidrule(lr){8-10}
%     \cmidrule(lr){11-13}
%     \cmidrule(lr){14-16}
%     % \cmidrule(lr){17-19}
%     \cmidrule(lr){20-22}
%     % \cmidrule(lr){23-25}
%     \cmidrule(lr){26-28}
%     % \cmidrule(lr){29-31}
% \multicolumn{4}{l}{HT-Demucs (VDBGPO)} & 
%     8.3 & 9.0 & 10.3 & &&&
%     \textbf{\textit{9.0}} & \textbf{\textit{11.6}} & \textbf{\textit{12.8}} & 
%     \textbf{\textit{11.2}} & \textbf{\textit{12.4}} & \textbf{\textit{14.1}} & &&& 
%     1.5 & 2.4 & 4.4 & &&&
%     0.2 & 1.7 & 2.3
% \\
% \multicolumn{4}{l}{Spleeter (VDBPO)} & 
%     6.0 & 7.0 & 7.7 & &&&
%     5.6 & 6.9 & 8.6 & 
%     5.2 & 6.7 & 8.8 & &&& 
%     &&& &&&
%     0.0 & 0.7 & 1.7
% \\
% \midrule

% \multicolumn{4}{l}{Oracle IBM} & 10.6 & 12.0 & 12.4 & 8.6 & 9.9 & 10.8 & 7.7 & 9.4 & 10.3 & 6.6 & 7.9 & 9.9 & 3.4 & 4.3 & 6.2 & 3.9 & 5.8 & 7.3 & 5.0 & 6.1 & 7.5 & 3.4 & 4.3 & 6.1 & 4.1 & 5.2 & 5.5 \\

% \multicolumn{4}{l}{Oracle IRM} & 10.0 & 11.3 & 11.9 & 8.0 & 9.3 & 10.1 & 7.0 & 8.5 & 9.5 & 6.0 & 7.4 & 9.3 & 3.0 & 4.2 & 5.7 & 3.5 & 5.6 & 6.9 & 4.6 & 5.8 & 6.9 & 3.1 & 4.4 & 5.8 & 3.9 & 4.9 & 5.2 \\
\bottomrule
\end{tabularx}

==> tables/vdbo.tex <==

    \begin{tabularx}{\columnwidth}{XS[table-format=-2.1]S[table-format=-2.1]S[table-format=-2.1]S[table-format=-2.1]}
        \toprule
        % & \multicolumn{4}{c}{\textbf{Median SNR (dB)}} \\
        % \cmidrule{2-5} 
        \textbf{Model} \hfill \textbf{Median SNR (dB):} & {\textbf{Vocals}} & {\textbf{Drums}} & {\textbf{Bass}} & {\textbf{Other}} \\
        \midrule
        Bandit \cite{Watcharasupat2023GeneralizedBandsplitNeural} & \bfseries 9.1 & 9.9 & 10.6 & 6.4 \\
        HT-Demucs \cite{Rouard2023HybridTransformersMusic} & \bfseries 9.1 & \bfseries 11.0 & \bfseries 12.2 & \bfseries 7.3 \\
        Spleeter \cite{Hennequin2020SpleeterFastEfficient} & 7.4 & 6.6 & 6.8 & 5.0 \\
        \midrule
        Oracle IRM & 10.3 & 9.2 & 8.8 & 7.6\\
        \bottomrule
    \end{tabularx}
